Partial Quantifier Elimination With Learning

We consider a modification of the Quantifier Elimination (QE) problem called Partial QE (PQE). In PQE, only a small part of the formula is taken out of the scope of quantifiers. The appeal of PQE is that many verification problems, e.g. equivalence checking and model checking, reduce to PQE and the latter is much easier than complete QE. Earlier, we introduced a PQE algorithm based on the machinery of D-sequents. A D-sequent is a record stating that a clause is redundant in a quantified CNF formula in a specified subspace. To make this algorithm efficient, it is important to reuse learned D-sequents. However, reusing D-sequents is not as easy as conflict clauses in SAT-solvers because redundancy is a structural rather than a semantic property. Earlier, we modified the definition of D-sequents to enable their safe reusing. In this paper, we present a PQE algorithm based on new D-sequents. It is different from its predecessor in two aspects. First, the new algorithm can learn and reuse D-sequents. Second, it proves clauses redundant one by one and thus backtracks as soon as the current target clause is proved redundant in the current subspace. This makes the new PQE algorithm similar to a SAT-solver that backtracks as soon as just one clause is falsified. We show experimentally that the new PQE algorithm outperforms its predecessor.

==> d0iv_conq.tex <==
\section{Partial Quantifier Elimination By Branching} 
\label{sec:div_conq}
In this paper, we present \Apqe, a modification of
\apqe~\cite{fmcad13} that reuses D-sequents. In this section, to make
the exposition easier to follow, we relate the main features of
\apqe/\Apqe to Sections~\ref{sec:dseqs}-\ref{sec:reuse} where
the semantics of these features is explained. \apqe is recalled in
Section~\ref{sec:apqe}. \Apqe is introduced in Section~\ref{sec:Apqe}.


\Apqe is a branching algorithm. It proves redundancy of $X$-clauses in
subspaces (i.e. ``conditionally'') and merges the results of different
branches to prove the unconditional redundancy of $X$-clauses.  \Apqe
operates on D-sequents. The latter is a record stating that an
$X$-clause is redundant in a specified subspace.  In
Section~\ref{sec:dseqs}, we give a definition of a D-sequent and
explain how this definition is different from that of~\cite{fmcad13}.

There are two ways for \Apqe \,to produce D-sequents. First, if
proving redundancy of a clause is trivial, \Apqe generates a so-called
atomic D-sequent.  The atomic D-sequents are introduced in
Section~\ref{sec:atom_dseqs}. Second, a new D-sequent can be produced
from two D-sequents by a resolution-like operation called
\ti{join}. This operation is described in
Section~\ref{sec:join_dseqs}. It is used by \Apqe when merging results
obtained in different branches.  A D-sequent generated by \Apqe in one
subspace can be reused in another subspace.  In
Section~\ref{sec:reuse}, we describe the condition under which a
D-sequent can be safely reused.





==> f11ootnote.tex <==
In the current context, a boundary point \pnt{p} is a full assignment
(\pnt{x},\pnt{y}) to $X \cup Y$ that falsifies $C$ but satisfies $(F_1
\cup F_2) \setminus \s{C}$. The boundary point \pnt{p} is called
removable if there is a clause $B(Y)$ implied by $F_1 \wedge F_2$ that
is falsified by \pnt{p}. Adding $B$ to $F_1 \wedge F_2$
eliminates \pnt{p} as a boundary point. $C$ is redundant in
\prob{X}{F_1 \wedge F_2} if no removable boundary point exists.


==> f1ootnote.tex <==
Let \pnt{s} denote a full assignment to $S$. In~\cite{mc_no_inv}, we
assume that $\forall \pnt{s}$, \mbox{$T(\pnt{s},\pnt{s})=1$}. So \ks
can ``stutter'' by staying in the current state \pnt{s}. If this is
not the case, one can introduce stuttering by adding to $T$ a
combinational variable $v$.  The modified \ks works as before if $v=1$
and stutters if $v=0$.


==> f6ootnote.tex <==
As we mentioned in Subsection~\ref{ssec:lim_lrn}, \Bpqe partitions the
initial PQE problem into smaller PQE problems where only one clause is
taken out of the scope of quantifiers. \Bpqe reuses only D-sequents
of \ti{this} clause.  The last column of Table~\ref{tbl:mc} gives the
total number of additional clauses \Bpqe had to prove redundant in
deeper subspaces without reusing their D-sequents.


==> f8ootnote.tex <==
As mentioned earlier, redundancy is a structural property of formula
$F$ (regardless of whether or not $F$ has quantifiers). It holds only
for a \ti{subset} of formulas logically equivalent to $F$.


==> f9ootnote.tex <==
We will introduce the notion of consistent D-sequents later, see
Definition~\ref{def:cons_dseqs}. Consistency of D-sequents in
Proposition~\ref{prop:dseq_third_kind} means that $C_1,\dots,C_k$ are
redundant together in subspace
\pnt{q}=$\bigcup\limits_{i=1}^{i=k}\ppnt{q}{i}$. So clause $C$ is
blocked at variable $v$ in subspace \pnt{q}.


==> r4elax_dseqs.tex <==
%\section{A Few Useful Procedures For Transforming D-sequents}
\section{Relaxing the order constraint of a D-sequent}
\label{app:relax}

This section describes a transformation used by \Apqe when merging the
results of two branches (by applying the join operation). To guarantee
that a new D-sequent $S$ is consistent with the D-sequents generated
earlier, one may need to relax the order constraint of $S$. (This is
achieved by relaxing the order constraints of the parents of $S$.)

Below, we give two propositions showing how one can make a D-sequent
$S$ ``more robust''. Proposition~\ref{prop:subst} introduces a
transformation that removes a clause from the order constraint of $S$
possibly adding to the latter some other clauses and making the
conditional of $S$ longer. Proposition~\ref{prop:mak_rob} shows that
by repeatedly applying this transformation one can remove a clause
from the order constraint of $S$ \ti{without} adding any other
clauses.

%
% Proposition: subsitutution
%
\begin{proposition}
  \label{prop:subst}  
Let \prob{X}{F} be an \ecnf formula.  Let \oDs{\pnt{q'}}{H'}{C'} and
$(\pnt{q''}$, $H'')$ $\rightarrow C''$ be consistent D-sequents (see
Definition~\ref{def:cons_dseqs}). Let $C''$ be in $H'$. Then D-sequent
\ods{q}{H}{C'} holds where $\pnt{q} = \pnt{q'} \cup \pnt{q''}$ and $H
= (H' \setminus \s{C''}) \cup H''$.
\end{proposition}



%
%  Proposition: making D-sequent more robust
%
\begin{proposition}
\label{prop:mak_rob}
Let \prob{X}{F} be an \ecnf formula and $(\ppnt{q}{1},H_1)$
$\rightarrow C_1$,$\dots$, $(\ppnt{q}{n}$, $H_k)$$\rightarrow C_k$ be
consistent D-sequents where $H_i \subseteq \s{C_1,\dots,C_k}$,
$i=1,\dots,k$. Assume, for the sake of simplicity, that the numbering
order is consistent with the order constraints of these
D-sequents. Let $C_m$ be in $H_i$.  Then, by repeatedly applying the
transformation of Proposition~\ref{prop:subst}, one can produce
D-sequent \ods{q}{H_i \setminus \s{C_m}}{C_i} where
$\ppnt{q}{i}~\subseteq~\pnt{q} \subseteq \ppnt{q}{i} \cup
\bigcup\limits_{j=m}^{j=k} \ppnt{q}{j}$.
\end{proposition}


